DAM-Seg: Anatomically accurate cardiac segmentation using Dense Associative Networks

Deep learning-based cardiac segmentation has seen significant advancements over the years. Many studies have tackled the challenge of anatomically incorrect segmentation predictions by introducing auxiliary modules. These modules either post-process segmentation outputs or enforce consistency between specific points to ensure anatomical correctness. However, such approaches often increase network complexity, require separate training for these modules, and may lack robustness in scenarios with poor visibility. To address these limitations, we propose a novel transformer-based architecture that leverages dense associative networks to learn and retain specific patterns inherent to cardiac inputs. Unlike traditional methods, our approach restricts the network to memorize a limited set of patterns. During forward propagation, a weighted sum of these patterns is used to enforce anatomical correctness in the output. Since these patterns are input-independent, the model demonstrates enhanced robustness, even in cases with poor visibility. The proposed pipeline was evaluated on two publicly available datasets, CAMUS and CardiacNet. Experimental results indicate that our model consistently outperforms baseline approaches across all metrics, highlighting its effectiveness and reliability for cardiac segmentation tasks.

==> Reference.tex <==
@article{adiga2024anatomically,
  title={Anatomically-aware uncertainty for semi-supervised image segmentation},
  author={Adiga, Sukesh and Dolz, Jose and Lombaert, Herve},
  journal={Medical Image Analysis},
  volume={91},
  pages={103011},
  year={2024},
  publisher={Elsevier}
}

@article{van2024towards,
  title={Towards Robust Cardiac Segmentation using Graph Convolutional Networks},
  author={Van De Vyver, Gilles and Thomas, Sarina and Ben-Yosef, Guy and Olaisen, Sindre Hellum and Dalen, H{\aa}vard and L{\o}vstakken, Lasse and Smistad, Erik},
  journal={IEEE Access},
  year={2024},
  publisher={IEEE}
}

@article{wyburd2024anatomically,
  title={Anatomically plausible segmentations: Explicitly preserving topology through prior deformations},
  author={Wyburd, Madeleine K and Dinsdale, Nicola K and Jenkinson, Mark and Namburete, Ana IL},
  journal={Medical Image Analysis},
  pages={103222},
  year={2024},
  publisher={Elsevier}
}

@article{gao2023anatomy,
  title={An anatomy-aware framework for automatic segmentation of parotid tumor from multimodal MRI},
  author={Gao, Yifan and Dai, Yin and Liu, Fayu and Chen, Weibing and Shi, Lifu},
  journal={Computers in Biology and Medicine},
  volume={161},
  pages={107000},
  year={2023},
  publisher={Elsevier}
}

@article{von2023anatomically,
  title={Anatomically-guided deep learning for left ventricle geometry generation with uncertainty quantification based on short-axis MR images},
  author={Von Zuben, Andre and Perotti, Luigi E and Viana, Felipe AC},
  journal={Engineering Applications of Artificial Intelligence},
  volume={121},
  pages={106012},
  year={2023},
  publisher={Elsevier}
}



@misc{polynomial_DAM,
      title={Dense Associative Memory for Pattern Recognition}, 
      author={Dmitry Krotov and John J Hopfield},
      year={2016},
      eprint={1606.01164},
      archivePrefix={arXiv},
      primaryClass={cs.NE},
      url={https://arxiv.org/abs/1606.01164}, 
}

@article{exponential_Demircigil,
   title={On a Model of Associative Memory with Huge Storage Capacity},
   volume={168},
   ISSN={1572-9613},
   url={http://dx.doi.org/10.1007/s10955-017-1806-y},
   DOI={10.1007/s10955-017-1806-y},
   number={2},
   journal={Journal of Statistical Physics},
   publisher={Springer Science and Business Media LLC},
   author={Demircigil, Mete and Heusel, Judith and Löwe, Matthias and Upgang, Sven and Vermet, Franck},
   year={2017},
   month=may, pages={288–299} }

@misc{SA_update,
      title={Hopfield Networks is All You Need}, 
      author={Hubert Ramsauer and Bernhard Schäfl and Johannes Lehner and Philipp Seidl and Michael Widrich and Thomas Adler and Lukas Gruber and Markus Holzleitner and Milena Pavlović and Geir Kjetil Sandve and Victor Greiff and David Kreil and Michael Kopp and Günter Klambauer and Johannes Brandstetter and Sepp Hochreiter},
      year={2021},
      eprint={2008.02217},
      archivePrefix={arXiv},
      primaryClass={cs.NE},
      url={https://arxiv.org/abs/2008.02217}, 
}

@misc{DeepRC,
      title={Modern Hopfield Networks and Attention for Immune Repertoire Classification}, 
      author={Michael Widrich and Bernhard Schäfl and Hubert Ramsauer and Milena Pavlović and Lukas Gruber and Markus Holzleitner and Johannes Brandstetter and Geir Kjetil Sandve and Victor Greiff and Sepp Hochreiter and Günter Klambauer},
      year={2020},
      eprint={2007.13505},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2007.13505}, 
}

@misc{universal_networks,
      title={Universal Hopfield Networks: A General Framework for Single-Shot Associative Memory Models}, 
      author={Beren Millidge and Tommaso Salvatori and Yuhang Song and Thomas Lukasiewicz and Rafal Bogacz},
      year={2022},
      eprint={2202.04557},
      archivePrefix={arXiv},
      primaryClass={cs.NE},
      url={https://arxiv.org/abs/2202.04557}, 
}

@misc{dpt,
      title={Vision Transformers for Dense Prediction}, 
      author={René Ranftl and Alexey Bochkovskiy and Vladlen Koltun},
      year={2021},
      eprint={2103.13413},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/2103.13413}, 
}

@article{RV_segmentation,
  title={Right ventricle segmentation from cardiac MRI: a collation study},
  author={Petitjean, Caroline and Zuluaga, Maria A and Bai, Wenjia and Dacher, Jean-Nicolas and Grosgeorge, Damien and Caudron, J{\'e}r{\^o}me and Ruan, Su and Ayed, Ismail Ben and Cardoso, M Jorge and Chen, Hsiang-Chou and others},
  journal={Medical image analysis},
  volume={19},
  number={1},
  pages={187--202},
  year={2015},
  publisher={Elsevier}
}

@misc{fcn,
      title={Fully Convolutional Networks for Semantic Segmentation}, 
      author={Jonathan Long and Evan Shelhamer and Trevor Darrell},
      year={2015},
      eprint={1411.4038},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/1411.4038}, 
}

@misc{cardiac_fcn,
      title={A Fully Convolutional Neural Network for Cardiac Segmentation in Short-Axis MRI}, 
      author={Phi Vu Tran},
      year={2017},
      eprint={1604.00494},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/1604.00494}, 
}

@ARTICLE{VAE_wrapping,
  author={Painchaud, Nathan and Skandarani, Youssef and Judge, Thierry and Bernard, Olivier and Lalande, Alain and Jodoin, Pierre-Marc},
  journal={IEEE Transactions on Medical Imaging}, 
  title={Cardiac Segmentation With Strong Anatomical Guarantees}, 
  year={2020},
  volume={39},
  number={11},
  pages={3703-3713},
  keywords={Shape;Image segmentation;Magnetic resonance imaging;Ultrasonic imaging;Three-dimensional displays;Neural networks;CNN;variational autoencoder;cardiac segmentation;MRI;ultrasound},
  doi={10.1109/TMI.2020.3003240}}

@ARTICLE{GCN,
  author={Vyver, Gilles Van De and Thomas, Sarina and Ben-Yosef, Guy and Olaisen, Sindre Hellum and Dalen, Håvard and Løvstakken, Lasse and Smistad, Erik},
  journal={IEEE Access}, 
  title={Toward Robust Cardiac Segmentation Using Graph Convolutional Networks}, 
  year={2024},
  volume={12},
  number={},
  pages={33876-33888},
  keywords={Image segmentation;Decoding;Computer architecture;Ultrasonic imaging;Convolutional neural networks;Real-time systems;Solid modeling;Cardiology;Graph neural networks;Robust control;Cardiac segmentation;graph convectional network;robust segmentation;ultrasound},
  doi={10.1109/ACCESS.2024.3373046}}

@article{hopfield_orig,
  title={Neural networks and physical systems with emergent collective computational abilities.},
  author={Hopfield, John J},
  journal={Proceedings of the national academy of sciences},
  volume={79},
  number={8},
  pages={2554--2558},
  year={1982},
  publisher={National Acad Sciences}
}

@misc{properties_nn,
      title={Intriguing properties of neural networks}, 
      author={Christian Szegedy and Wojciech Zaremba and Ilya Sutskever and Joan Bruna and Dumitru Erhan and Ian Goodfellow and Rob Fergus},
      year={2014},
      eprint={1312.6199},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/1312.6199}, 
}

@misc{nn_easily,
      title={Deep Neural Networks are Easily Fooled: High Confidence Predictions for Unrecognizable Images}, 
      author={Anh Nguyen and Jason Yosinski and Jeff Clune},
      year={2015},
      eprint={1412.1897},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/1412.1897}, 
}

@article{camus,
  title={Deep Learning for Segmentation Using an Open Large-Scale Dataset in 2D Echocardiography},
  author={Sarah Leclerc and Erik Smistad and Jo{\~a}o Pedrosa and Andreas {\O}stvik and Fr{\'e}d{\'e}ric Cervenansky and Florian Espinosa and Torvald Espeland and Erik Andreas Rye Berg and Pierre-Marc Jodoin and Thomas Grenier and Carole Lartizien and Jan D’hooge and Lasse L{\o}vstakken and Olivier Bernard},
  journal={IEEE Transactions on Medical Imaging},
  year={2019},
  volume={38},
  pages={2198-2210},
  url={https://api.semanticscholar.org/CorpusID:73510235}
}

@ARTICLE{displacement_aware,
  author={Li, Kang and Zhu, Yu and Yu, Lequan and Heng, Pheng-Ann},
  journal={IEEE Transactions on Medical Imaging}, 
  title={A Dual Enrichment Synergistic Strategy to Handle Data Heterogeneity for Domain Incremental Cardiac Segmentation}, 
  year={2024},
  volume={43},
  number={6},
  pages={2279-2290},
  keywords={Shape;Data models;Heart;Training data;Data privacy;Computational modeling;Robustness;Domain incremental learning;cardiac image segmentation;cardiac data heterogeneity},
  doi={10.1109/TMI.2024.3364240}}

@INPROCEEDINGS{cross_domain,
  author={Cai, Zhuotong and Xin, Jingmin and Dong, Siyuan and Onofrey, John A. and Zheng, Nanning and Duncan, James S.},
  booktitle={ICASSP 2024 - 2024 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={Symmetric Consistency with Cross-Domain Mixup for Cross-Modality Cardiac Segmentation}, 
  year={2024},
  volume={},
  number={},
  pages={1536-1540},
  keywords={Training;Heart;Image segmentation;Adaptation models;Statistical analysis;Annotations;Signal processing;Mixup;Cross-modality;Cardiac Segmentation;Unsupervised Domain Adaptation},
  doi={10.1109/ICASSP48485.2024.10447304}}


@misc{memformer,
      title={Memformer: A Memory-Augmented Transformer for Sequence Modeling}, 
      author={Qingyang Wu and Zhenzhong Lan and Kun Qian and Jing Gu and Alborz Geramifard and Zhou Yu},
      year={2022},
      eprint={2010.06891},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2010.06891}, 
}

@misc{rate,
      title={Recurrent Action Transformer with Memory}, 
      author={Egor Cherepanov and Alexey Staroverov and Dmitry Yudin and Alexey K. Kovalev and Aleksandr I. Panov},
      year={2024},
      eprint={2306.09459},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2306.09459}, 
}

@article{CANet,
   title={CANet: An Unsupervised Intrusion Detection System for High Dimensional CAN Bus Data},
   volume={8},
   ISSN={2169-3536},
   url={http://dx.doi.org/10.1109/ACCESS.2020.2982544},
   DOI={10.1109/access.2020.2982544},
   journal={IEEE Access},
   publisher={Institute of Electrical and Electronics Engineers (IEEE)},
   author={Hanselmann, Markus and Strauss, Thilo and Dormann, Katharina and Ulmer, Holger},
   year={2020},
   pages={58194–58205} }

@misc{nnUnet,
      title={nnU-Net: Self-adapting Framework for U-Net-Based Medical Image Segmentation}, 
      author={Fabian Isensee and Jens Petersen and Andre Klein and David Zimmerer and Paul F. Jaeger and Simon Kohl and Jakob Wasserthal and Gregor Koehler and Tobias Norajitra and Sebastian Wirkert and Klaus H. Maier-Hein},
      year={2018},
      eprint={1809.10486},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/1809.10486}, 
}

@misc{extended_nnunet,
      title={Extending nnU-Net is all you need}, 
      author={Fabian Isensee and Constantin Ulrich and Tassilo Wald and Klaus H. Maier-Hein},
      year={2022},
      eprint={2208.10791},
      archivePrefix={arXiv},
      primaryClass={eess.IV},
      url={https://arxiv.org/abs/2208.10791}, 
}

@misc{unet,
      title={U-Net: Convolutional Networks for Biomedical Image Segmentation}, 
      author={Olaf Ronneberger and Philipp Fischer and Thomas Brox},
      year={2015},
      eprint={1505.04597},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/1505.04597}, 
}

@misc{cardiacnet,
      title={GraphEcho: Graph-Driven Unsupervised Domain Adaptation for Echocardiogram Video Segmentation}, 
      author={Jiewen Yang and Xinpeng Ding and Ziyang Zheng and Xiaowei Xu and Xiaomeng Li},
      year={2023},
      eprint={2309.11145},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/2309.11145}, 
}

@misc{largeassociativememoryproblem,
      title={Large Associative Memory Problem in Neurobiology and Machine Learning}, 
      author={Dmitry Krotov and John Hopfield},
      year={2021},
      eprint={2008.06996},
      archivePrefix={arXiv},
      primaryClass={q-bio.NC},
      url={https://arxiv.org/abs/2008.06996}, 
}
